The Cactus Group Property for Ordinal Sums of Disjoint Unions of Chains

We study the action of Bender-Knuth involutions on linear extensions of posets and identify LE-cactus posets, i.e. those for which the cactus relations hold. It was conjectured in \cite{chiang2023bender} that d-complete posets are LE-cactus. Among the non-d-complete posets that are LE-cactus, one notable family is ordinal sums of antichains. In this paper, we characterize the LE-cactus posets in a more general family, namely ordinal sums of disjoint unions of chains.

==> tikz.tex <==
% SYT-Ferrer

% \draw[black, thick] (0,0) -- (2,0);
% \draw[black, thick] (0,1) -- (3,1);
% \draw[black, thick] (0,2) -- (3,2);
% \draw[black, thick] (0,0) -- (0,2);
% \draw[black, thick] (1,0) -- (1,2);
% \draw[black, thick] (2,0) -- (2,2);
% \draw[black, thick] (3,1) -- (3,2);

% \draw (0.5,0.5) node[anchor=center] {\huge 2};
% \draw (1.5,0.5) node[anchor=center] {\huge 4};
% \draw (0.5,1.5) node[anchor=center] {\huge 1};
% \draw (1.5,1.5) node[anchor=center] {\huge 3};
% \draw (2.5,1.5) node[anchor=center] {\huge 5};

% \draw [-{Stealth[scale = 2]}](4,1) -- (6,1);

% \filldraw[black] (9,0) circle (2pt);
% \filldraw[black] (8,1) circle (2pt);
% \filldraw[black] (10,1) circle (2pt);
% \filldraw[black] (7,2) circle (2pt);
% \filldraw[black] (9,2) circle (2pt);

% \draw[black, thick] (9,0) -- (7,2);
% \draw[black, thick] (9,0) -- (10,1);
% \draw[black, thick] (9,2) -- (10,1);
% \draw[black, thick] (9,2) -- (8,1);


% \draw (9,-0.5) node[anchor=center] {\huge 1};
% \draw (10,0.5) node[anchor=center] {\huge 2};
% \draw (8,0.5) node[anchor=center] {\huge 3};
% \draw (9,2.5) node[anchor=center] {\huge 4};
% \draw (7,2.5) node[anchor=center] {\huge 5};



%%%%%%%%%%%------------------%%%%%%%%%%%%%%%%

% ex-promotion

% \node (v1) [fill = gray,circle,scale=1,anchor=center] at (0,0) {\textcolor{white}{1}};
% \node (v2) [fill = gray,circle,scale=1,anchor=center] at (2,0) {\textcolor{white}{3}};
% \node (v3) [fill = gray,circle,scale=1,anchor=center] at (-1,2) {\textcolor{white}{2}};
% \node (v4) [fill = gray,circle,scale=1,anchor=center] at (1,2) {\textcolor{white}{4}};
% \node (v5) [fill = gray,circle,scale=1,anchor=center] at (3,2) {\textcolor{white}{6}};
% \node (v6) [fill = gray,circle,scale=1,anchor=center] at (0,4) {\textcolor{white}{5}};
% \node (v7) [fill = gray,circle,scale=1,anchor=center] at (2,4) {\textcolor{white}{7}};

% \draw[black, line width=1pt] (v1) -- (v3);
% \draw[black, line width=1pt] (v1) -- (v4);
% \draw[black, line width=1pt] (v1) -- (v5);
% \draw[black, line width=1pt] (v2) -- (v4);
% \draw[black, line width=1pt] (v2) -- (v5);
% \draw[black, line width=1pt] (v3) -- (v6);
% \draw[black, line width=1pt] (v4) -- (v6);
% \draw[black, line width=1pt] (v4) -- (v7);
% \draw[black, line width=1pt] (v5) -- (v7);




%%%%%-----------------%%%%%%



% D_3_posets


% \node (v4) [fill = black,circle,scale=1,anchor=center] at (4,0) {};
% \node (v5) [fill = black,circle,scale=1,anchor=center] at (4,2) {};
% \node (v6) [fill = black,circle,scale=1,anchor=center] at (6,0) {};

% \draw[black, line width=1pt] (v4) -- (v5);

% \draw (5,-1.5) node[anchor=center, scale = 2] {$D_{(2,1)}$};




% \node (v7) [fill = black,circle,scale=1,anchor=center] at (10,0) {};
% \node (v8) [fill = black,circle,scale=1,anchor=center] at (12,0) {};
% \node (v9) [fill = black,circle,scale=1,anchor=center] at (14,0) {};

% \draw (12,-1.5) node[anchor=center, scale = 2] {$D_{(1,1,1)}$};





%%%%%%%%%% ---------------- %%%%%%%%%%%%%%

% pro-neck

% \node (v1) [fill = red,circle,scale=1,anchor=center] at (0,0) {\textcolor{white}{1}};
% \node (v2) [fill = red,circle,scale=1,anchor=center] at (0,2) {\textcolor{white}{3}};
% \node (v3) [fill = red,circle,scale=1,anchor=center] at (0,4) {\textcolor{white}{4}};
% \node (v4) [fill = red,circle,scale=1,anchor=center] at (0,6) {\textcolor{white}{7}};
% \node (v5) [fill = blue,circle,scale=1,anchor=center] at (2,0) {\textcolor{white}{5}};
% \node (v6) [fill = blue,circle,scale=1,anchor=center] at (2,2) {\textcolor{white}{8}};
% \node (v7) [fill = brown,circle,scale=1,anchor=center] at (4,0) {\textcolor{white}{2}};
% \node (v8) [fill = brown,circle,scale=1,anchor=center] at (4,2) {\textcolor{white}{6}};

% \draw[black, line width=1pt] (v1) -- (v2);
% \draw[black, line width=1pt] (v2) -- (v3);
% \draw[black, line width=1pt] (v3) -- (v4);
% \draw[black, line width=1pt] (v5) -- (v6);
% \draw[black, line width=1pt] (v7) -- (v8);


% \draw (2,-2) node[anchor=center, scale = 1.5] {$(\{\textcolor{red}{1},\textcolor{red}{3},\textcolor{red}{4},7\},\{\textcolor{red}{5},8\},\{\textcolor{red}{2},6\})$};


% \draw [-{Stealth[scale = 2]}](6,3) -- (8,3);
% \draw (7,3.5) node[anchor=center, scale = 1.5] {$\partial_5$};


% \draw [-{Stealth[scale = 2]}](6,-2) -- (8,-2);
% \draw (7,-1.5) node[anchor=center, scale = 1.5] {$(54321)$};


% \node (u1) [fill = red,circle,scale=1,anchor=center] at (10,0) {\textcolor{white}{2}};
% \node (u2) [fill = red,circle,scale=1,anchor=center] at (10,2) {\textcolor{white}{3}};
% \node (u3) [fill = red,circle,scale=1,anchor=center] at (10,4) {\textcolor{white}{5}};
% \node (u4) [fill = red,circle,scale=1,anchor=center] at (10,6) {\textcolor{white}{7}};
% \node (u5) [fill = blue,circle,scale=1,anchor=center] at (12,0) {\textcolor{white}{4}};
% \node (u6) [fill = blue,circle,scale=1,anchor=center] at (12,2) {\textcolor{white}{8}};
% \node (u7) [fill = brown,circle,scale=1,anchor=center] at (14,0) {\textcolor{white}{1}};
% \node (u8) [fill = brown,circle,scale=1,anchor=center] at (14,2) {\textcolor{white}{6}};

% \draw[black, line width=1pt] (u1) -- (u2);
% \draw[black, line width=1pt] (u2) -- (u3);
% \draw[black, line width=1pt] (u3) -- (u4);
% \draw[black, line width=1pt] (u5) -- (u6);
% \draw[black, line width=1pt] (u7) -- (u8);


% \draw (12,-2) node[anchor=center, scale = 1.5] {$(\{\textcolor{red}{5},\textcolor{red}{2},\textcolor{red}{3},7\},\{\textcolor{red}{4},8\},\{\textcolor{red}{1},6\})$};



%%%%%%%% --------------- %%%%%%%%%%%%

% eva-neck

% \node (v1) [fill = red,circle,scale=1,anchor=center] at (0,0) {\textcolor{white}{1}};
% \node (v2) [fill = red,circle,scale=1,anchor=center] at (0,2) {\textcolor{white}{3}};
% \node (v3) [fill = red,circle,scale=1,anchor=center] at (0,4) {\textcolor{white}{4}};
% \node (v4) [fill = red,circle,scale=1,anchor=center] at (0,6) {\textcolor{white}{7}};
% \node (v5) [fill = blue,circle,scale=1,anchor=center] at (2,0) {\textcolor{white}{5}};
% \node (v6) [fill = blue,circle,scale=1,anchor=center] at (2,2) {\textcolor{white}{8}};
% \node (v7) [fill = brown,circle,scale=1,anchor=center] at (4,0) {\textcolor{white}{2}};
% \node (v8) [fill = brown,circle,scale=1,anchor=center] at (4,2) {\textcolor{white}{6}};

% \draw[black, line width=1pt] (v1) -- (v2);
% \draw[black, line width=1pt] (v2) -- (v3);
% \draw[black, line width=1pt] (v3) -- (v4);
% \draw[black, line width=1pt] (v5) -- (v6);
% \draw[black, line width=1pt] (v7) -- (v8);


% \draw [-{Stealth[scale = 2]}](6,3) -- (8,3);


% \draw[black] (12,3) circle (2);
% \node (c1) [fill = red,circle,scale=1,anchor=center] at (12,5) {\textcolor{white}{1}};
% \node (c2) [fill = brown,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{2}};
% \node (c3) [fill = red,circle,scale=1,anchor=center] at (14,3) {\textcolor{white}{3}};
% \node (c4) [fill = red,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{4}};
% \node (c5) [fill = blue,circle,scale=1,anchor=center] at (12,1) {\textcolor{white}{5}};
% \node (c6) [fill = brown,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{6}};
% \node (c7) [fill = red,circle,scale=1,anchor=center] at (10,3) {\textcolor{white}{7}};
% \node (c8) [fill = blue,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{8}};


% \draw [-{Stealth[scale = 2]}](2,-2) -- (2,-4);
% \draw (1.5,-3) node[anchor=center, scale = 1.5] {$q_4$};


% \draw [-{Stealth[scale = 2]}](12,-2) -- (12,-4);
% \draw (13.25,-3) node[anchor=center, scale = 1.5] {$\left(\begin{smallmatrix} 
%     1 & 2 & 3 & 4 & 5\\
%     5 & 4 & 3 & 2 & 1
%     \end{smallmatrix}\right)$};


% \node (u1) [fill = red,circle,scale=1,anchor=center] at (0,-12) {\textcolor{white}{2}};
% \node (u2) [fill = red,circle,scale=1,anchor=center] at (0,-10) {\textcolor{white}{3}};
% \node (u3) [fill = red,circle,scale=1,anchor=center] at (0,-8) {\textcolor{white}{5}};
% \node (u4) [fill = red,circle,scale=1,anchor=center] at (0,-6) {\textcolor{white}{7}};
% \node (u5) [fill = blue,circle,scale=1,anchor=center] at (2,-12) {\textcolor{white}{1}};
% \node (u6) [fill = blue,circle,scale=1,anchor=center] at (2,-10) {\textcolor{white}{8}};
% \node (u7) [fill = brown,circle,scale=1,anchor=center] at (4,-12) {\textcolor{white}{4}};
% \node (u8) [fill = brown,circle,scale=1,anchor=center] at (4,-10) {\textcolor{white}{6}};

% \draw[black, line width=1pt] (u1) -- (u2);
% \draw[black, line width=1pt] (u2) -- (u3);
% \draw[black, line width=1pt] (u3) -- (u4);
% \draw[black, line width=1pt] (u5) -- (u6);
% \draw[black, line width=1pt] (u7) -- (u8);


% \draw [-{Stealth[scale = 2]}](6,-9) -- (8,-9);


% \draw[black] (12,-9) circle (2);
% \node (d1) [fill = red,circle,scale=1,anchor=center] at (12,-7) {\textcolor{white}{5}};
% \node (d2) [fill = brown,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ -9+sqrt(2) }) {\textcolor{white}{4}};
% \node (d3) [fill = red,circle,scale=1,anchor=center] at (14,-9) {\textcolor{white}{3}};
% \node (d4) [fill = red,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ -9-sqrt(2) }) {\textcolor{white}{2}};
% \node (d5) [fill = blue,circle,scale=1,anchor=center] at (12,-11) {\textcolor{white}{1}};
% \node (d6) [fill = brown,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ -9-sqrt(2) }) {\textcolor{white}{6}};
% \node (d7) [fill = red,circle,scale=1,anchor=center] at (10,-9) {\textcolor{white}{7}};
% \node (d8) [fill = blue,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ -9+sqrt(2) }) {\textcolor{white}{8}};



%%%%%% ----------- %%%%%%%

% min-non-cactus

% \node (v2) [fill = gray,circle,scale=1,anchor=center] at (4,0) {\textcolor{white}{2}};
% \node (v3) [fill = gray,circle,scale=1,anchor=center] at (6,0) {\textcolor{white}{3}};
% \node (v4) [fill = gray,circle,scale=1,anchor=center] at (2,0) {\textcolor{white}{1}};
% \node (v5) [fill = gray,circle,scale=1,anchor=center] at (4,2) {\textcolor{white}{4}};

% \draw[black, line width=1pt] (v2) -- (v5);
% \draw[black, line width=1pt] (v3) -- (v5);
% \draw[black, line width=1pt] (v4) -- (v5);



%%%%%% ------------ %%%%%%%%%%

% I-ex

% \node (v1) [fill = red,circle,scale=1,anchor=center] at (0,0) {\textcolor{white}{$p+1$}};
% \node (v2) [fill = red,circle,scale=1,anchor=center] at (0,2) {\textcolor{white}{$p+3$}};
% \node (v3) [fill = red,circle,scale=1,anchor=center] at (0,4) {\textcolor{white}{$p+4$}};
% \node (v4) [fill = red,circle,scale=1,anchor=center] at (0,6) {\textcolor{white}{$p+7$}};
% \node (v5) [fill = blue,circle,scale=1,anchor=center] at (2,2) {\textcolor{white}{$p+5$}};
% \node (v6) [fill = blue,circle,scale=1,anchor=center] at (2,4) {\textcolor{white}{$p+8$}};
% \node (v7) [fill = brown,circle,scale=1,anchor=center] at (4,2) {\textcolor{white}{$p+2$}};
% \node (v8) [fill = brown,circle,scale=1,anchor=center] at (4,4) {\textcolor{white}{$p+6$}};


% \node (p) [fill = gray,circle,scale=3,anchor=center] at (2,-3) {\textcolor{white}{$P$}};
% \node (q) [fill = gray,circle,scale=3,anchor=center] at (2,9) {\textcolor{white}{$Q$}};

% \draw[black, line width=1pt] (v1) -- (v2);
% \draw[black, line width=1pt] (v2) -- (v3);
% \draw[black, line width=1pt] (v3) -- (v4);
% \draw[black, line width=1pt] (v5) -- (v6);
% \draw[black, line width=1pt] (v7) -- (v8);


% \draw[black, line width=1pt] (p) -- (v1);
% \draw[black, line width=1pt] (p) -- (v5);
% \draw[black, line width=1pt] (p) -- (v7);

% \draw[black, line width=1pt] (q) -- (v4);
% \draw[black, line width=1pt] (q) -- (v6);
% \draw[black, line width=1pt] (q) -- (v8);



% \node (u1) [fill = red,circle,scale=1,anchor=center] at (10,0) {\textcolor{white}{1}};
% \node (u2) [fill = red,circle,scale=1,anchor=center] at (10,2) {\textcolor{white}{3}};
% \node (u3) [fill = red,circle,scale=1,anchor=center] at (10,4) {\textcolor{white}{4}};
% \node (u4) [fill = red,circle,scale=1,anchor=center] at (10,6) {\textcolor{white}{7}};
% \node (u5) [fill = blue,circle,scale=1,anchor=center] at (12,2) {\textcolor{white}{5}};
% \node (u6) [fill = blue,circle,scale=1,anchor=center] at (12,4) {\textcolor{white}{8}};
% \node (u7) [fill = brown,circle,scale=1,anchor=center] at (14,2) {\textcolor{white}{2}};
% \node (u8) [fill = brown,circle,scale=1,anchor=center] at (14,4) {\textcolor{white}{6}};

% \draw[black, line width=1pt] (u1) -- (u2);
% \draw[black, line width=1pt] (u2) -- (u3);
% \draw[black, line width=1pt] (u3) -- (u4);
% \draw[black, line width=1pt] (u5) -- (u6);
% \draw[black, line width=1pt] (u7) -- (u8);

% \draw [-{Stealth[scale = 2]}](6,3) -- (8,3);

% \draw (7,3.75) node[anchor=center, scale = 2] {$I$};



%%%%%%%%%% ----------- %%%%%%%%

% q_jk_neck

    % \draw[black] (12,3) circle (2);
    % \node (c1) [fill = red,circle,scale=1,anchor=center] at (12,5) {\textcolor{white}{7}};
% \node (c2) [fill = brown,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{6}};
% \node (c3) [fill = red,circle,scale=1,anchor=center] at (14,3) {\textcolor{white}{3}};
% \node (c4) [fill = red,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{4}};
% \node (c5) [fill = blue,circle,scale=1,anchor=center] at (12,1) {\textcolor{white}{5}};
% \node (c6) [fill = brown,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{1}};
% \node (c7) [fill = red,circle,scale=1,anchor=center] at (10,3) {\textcolor{white}{2}};
% \node (c8) [fill = blue,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{8}};


% \draw [-{Stealth[scale = 2]}](6,3) -- (8,3);


% \draw[black] (2,3) circle (2);
% \node (c1) [fill = red,circle,scale=1,anchor=center] at (2,5) {\textcolor{white}{1}};
% \node (c2) [fill = brown,circle,scale=1,anchor=center] at ({ 2+sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{2}};
% \node (c3) [fill = red,circle,scale=1,anchor=center] at (4,3) {\textcolor{white}{3}};
% \node (c4) [fill = red,circle,scale=1,anchor=center] at ({ 2+sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{4}};
% \node (c5) [fill = blue,circle,scale=1,anchor=center] at (2,1) {\textcolor{white}{5}};
% \node (c6) [fill = brown,circle,scale=1,anchor=center] at ({ 2-sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{6}};
% \node (c7) [fill = red,circle,scale=1,anchor=center] at (0,3) {\textcolor{white}{7}};
% \node (c8) [fill = blue,circle,scale=1,anchor=center] at ({ 2-sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{8}};



%%%%%%%%---------%%%%%%%%%


% s_n_necklace_ex

% \draw[black] (2,3) circle (2);
% \node (c1) [fill = red,circle,scale=1,anchor=center] at (2,5) {\textcolor{white}{1}};
% \node (c2) [fill = brown,circle,scale=1,anchor=center] at ({ 2+sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{4}};
% \node (c3) [fill = red,circle,scale=1,anchor=center] at (4,3) {\textcolor{white}{2}};
% \node (c4) [fill = red,circle,scale=1,anchor=center] at ({ 2+sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{6}};
% \node (c5) [fill = blue,circle,scale=1,anchor=center] at (2,1) {\textcolor{white}{7}};
% \node (c6) [fill = brown,circle,scale=1,anchor=center] at ({ 2-sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{3}};
% \node (c7) [fill = red,circle,scale=1,anchor=center] at (0,3) {\textcolor{white}{8}};
% \node (c8) [fill = blue,circle,scale=1,anchor=center] at ({ 2-sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{5}};


% \draw [-{Stealth[scale = 2]}](6,3) -- (8,3);
% \draw (7,3.5) node[anchor=center, scale = 1.5] {$(13284)$};

% \draw[black] (12,3) circle (2);
% \node (c1) [fill = red,circle,scale=1,anchor=center] at (12,5) {\textcolor{white}{3}};
% \node (c2) [fill = brown,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{1}};
% \node (c3) [fill = red,circle,scale=1,anchor=center] at (14,3) {\textcolor{white}{8}};
% \node (c4) [fill = red,circle,scale=1,anchor=center] at ({ 12+sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{6}};
% \node (c5) [fill = blue,circle,scale=1,anchor=center] at (12,1) {\textcolor{white}{7}};
% \node (c6) [fill = brown,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ 3-sqrt(2) }) {\textcolor{white}{2}};
% \node (c7) [fill = red,circle,scale=1,anchor=center] at (10,3) {\textcolor{white}{4}};
% \node (c8) [fill = blue,circle,scale=1,anchor=center] at ({ 12-sqrt(2) },{ 3+sqrt(2) }) {\textcolor{white}{5}};
